Mcity Data Collection for Automated Vehicles Study

The main goal of this paper is to introduce the data collection effort at Mcity targeting automated vehicle development. We captured a comprehensive set of data from a set of perception sensors (Lidars, Radars, Cameras) as well as vehicle steering/brake/throttle inputs and an RTK unit. Two in-cabin cameras record the human driver's behaviors for possible future use. The naturalistic driving on selected open roads is recorded at different time of day and weather conditions. We also perform designed choreography data collection inside the Mcity test facility focusing on vehicle to vehicle, and vehicle to vulnerable road user interactions which is quite unique among existing open-source datasets. The vehicle platform, data content, tags/labels, and selected analysis results are shown in this paper.

==> codes_backup.tex <==
\begin{figure*}[!b]
\centering
  \begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[width = \linewidth]{Figures/NDS_Samples/1.jpg}
    %\caption{First image}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[width = \linewidth]{Figures/NDS_Samples/2.jpg}
    %\caption{First image}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[width = \linewidth]{Figures/NDS_Samples/3.jpg}
    %\caption{First image}
  \end{subfigure}%
\\ \vspace{3pt}
  \begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[width = \linewidth]{Figures/NDS_Samples/4.jpg}
    %\caption{First image}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[width = \linewidth]{Figures/NDS_Samples/5.jpg}
    %\caption{First image}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[width = \linewidth]{Figures/NDS_Samples/6.jpg}
    %\caption{First image}
  \end{subfigure}%
\\ \vspace{3pt}
  \begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[width = \linewidth]{Figures/NDS_Samples/7.jpg}
    %\caption{First image}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[width = \linewidth]{Figures/NDS_Samples/8.jpg}
    %\caption{First image}
  \end{subfigure}%
  \hfill
  \begin{subfigure}{.33\linewidth}
    \centering
    \includegraphics[width = \linewidth]{Figures/NDS_Samples/9.jpg}
    %\caption{First image}
  \end{subfigure}%
\caption{Sampled images (from front 60$^o$FOV camera) collected on open roads. Left to right, top to bottom: highway, dawn, tunnel, snow, rainy, foggy, night, high speed local road, bridge.}
\label{nds_samples}
\end{figure*}




\clearpage
\begin{figure*}[t]
\centering
\begin{subfigure}{.36\columnwidth}
\centering
\includegraphics[width=.9\textwidth]{Figures/v_v_interaction/1.pdf}%
\caption{Low speed merge. Vehicle in the ramp merges into the main road.}
\end{subfigure}
\begin{subfigure}{.36\columnwidth}
\centering
\includegraphics[width=.9\textwidth]{Figures/v_v_interaction/2.pdf}%
\caption{Vehicle cuts into the lane at certain speed and longitudinal displacement.}
\end{subfigure}
\begin{subfigure}{.36\columnwidth}
\centering
\includegraphics[width=.9\textwidth]{Figures/v_v_interaction/3.pdf}%
\caption{Vehicle parked on the road, driver's seat door ajar.\\}
\end{subfigure}
\begin{subfigure}{.36\columnwidth}
\centering
\includegraphics[width=.9\textwidth]{Figures/v_v_interaction/4.pdf}%
\caption{Passes parked vehicle, goes over lane line if necessary.\\}
\end{subfigure}
\vspace{.1cm}
\begin{subfigure}{.4\columnwidth}
\centering
\includegraphics[width=.8\textwidth]{Figures/v_v_interaction/5.pdf}%
\caption{Vehicle starts up from road side.}
\end{subfigure}
\begin{subfigure}{.4\columnwidth}
\centering
\includegraphics[width=.8\textwidth]{Figures/v_v_interaction/6.pdf}%
\caption{Vehicle exits inclined parking spot, merges into the main road.}
\end{subfigure}
\begin{subfigure}{.4\columnwidth}
\centering
\includegraphics[width=.8\textwidth]{Figures/v_v_interaction/7.pdf}%
\caption{Vehicle performs unprotected right turn.}
\end{subfigure}
\begin{subfigure}{.4\columnwidth}
\centering
\includegraphics[width=.8\textwidth]{Figures/v_v_interaction/8.pdf}%
\caption{Vehicle performs unprotected left turn.}
\end{subfigure}
\begin{subfigure}{.4\columnwidth}
\centering
\includegraphics[width=.8\textwidth]{Figures/v_v_interaction/9.pdf}%
\caption{Vehicle enters a round about.}
\end{subfigure}
\caption{Designed choreography for the vehicle to vehicle interaction data collection inside MCity. We swapped the roles of the two vehicles in the collection (except for the door ajar scenario). We recorded both normal and abnormal drivings (yielding/not yielding to rights of way), and we repeated three times for each data collection run.}
\label{v_v_interactions}
\end{figure*}


\begin{figure*}[t]
\centering
\begin{subfigure}{.6\columnwidth}
\centering
\includegraphics[width=.8\textwidth]{Figures/v_pb_interaction/1.pdf}%
\caption{Vehicle straight movement, interacts with pedestrian/bicyclist at crosswalk.}
\end{subfigure}
\hfill
\vspace{.1cm}
\begin{subfigure}{.6\columnwidth}
\centering
\includegraphics[width=.8\textwidth]{Figures/v_pb_interaction/2.pdf}%
\caption{Vehicle right turn, interacts with pedestrian/bicyclist at crosswalk.}
\end{subfigure}
\hfill
\vspace{.1cm}
\begin{subfigure}{.6\columnwidth}
\centering
\includegraphics[width=.8\textwidth]{Figures/v_pb_interaction/3.pdf}%
\caption{Vehicle left turn, interacts with pedestrian/bicyclist at crosswalk.}
\end{subfigure}
\hfill
\vspace{.1cm}
\begin{subfigure}{.6\columnwidth}
\centering
\includegraphics[width=.8\textwidth]{Figures/v_pb_interaction/4.pdf}%
\caption{Vehicle follows pedestrian/bicyclist on the road.}
\end{subfigure}
\hfill
\vspace{.1cm}
\begin{subfigure}{.6\columnwidth}
\centering
\includegraphics[width=.8\textwidth]{Figures/v_pb_interaction/5.pdf}%
\caption{Vehicle passes pedestrian/bicyclist on the road.}
\end{subfigure}
\hfill
\vspace{.1cm}
\begin{subfigure}{.6\columnwidth}
\centering
\includegraphics[width=.8\textwidth]{Figures/v_pb_interaction/6.pdf}%
\caption{Vehicle follows pedestrian/bicyclist on the road. Pedestrian/bicyclist yields to the vehicle and let it pass.}
\end{subfigure}
\hfill
\vspace{.1cm}
\begin{subfigure}{.6\columnwidth}
\centering
\includegraphics[width=.8\textwidth]{Figures/v_pb_interaction/7.pdf}%
\caption{Pedestrian/Bicyclist emerges from behind occlusion.}
\end{subfigure}
\hfill
\vspace{.1cm}
\begin{subfigure}{.6\columnwidth}
\centering
\includegraphics[width=.8\textwidth]{Figures/v_pb_interaction/8.pdf}%
\caption{Vehicle enters round about, interacts with pedestrian/bicyclist at crosswalk.}
\end{subfigure}
\hfill
\vspace{.1cm}
\begin{subfigure}{.6\columnwidth}
\centering
\includegraphics[width=.8\textwidth]{Figures/v_pb_interaction/9.pdf}%
\caption{Vehicle exits round about, interacts with pedestrian/bicyclist at crosswalk.}
\end{subfigure}
\hfill
\vspace{.1cm}
\caption{We collected both obeying and disobeying rights of way for scenario (a~c) and (g-i). We also repeated three times for each scenario collection. }
\label{v_pb_interactions}
\end{figure*}



\begin{table}[t]
    \centering
    \caption{A summary of different driving scenarios recorded in the open roads data collection.}
    \label{7_case_summary}
    \begin{tabular}{lcccc}
    \hline
    \hline 
    Scenario    &\begin{tabular}[c]{@{}l@{}} \shortstack{Size\\($\#$)}  \end{tabular}    
                &\begin{tabular}[c]{@{}l@{}} \shortstack{Total\\Time (min)}  \end{tabular}
                &\begin{tabular}[c]{@{}l@{}} \shortstack{Min\\Time (s)}  \end{tabular}
                &\begin{tabular}[c]{@{}l@{}} \shortstack{Max\\Time (s)}  \end{tabular}\\
    \hline
    \textbf{Left turn}          &117               &20.383                   &1                 &74          \\
    \textbf{Left LC}            &216               &15.700                   &1                 &33          \\
    \textbf{Highway enter}      &32               &3.583                   &2                 &25          \\
    \textbf{Right turn}         &148               &21.833                   &1                 &35          \\
    \textbf{Right LC}           &187               &13.267                   &1                 &44          \\
    \textbf{Highway exit}       &33               &3.200                   &2                 &40          \\
    \textbf{Lane keeping}       &812                  &1207                   &1                    &1220             \\
    \hline
    \multicolumn{5}{p{.9\columnwidth}}{\textbf{Note: } In the collection runs the human driver is required to implement the turning signal strictly following the traffic rules. We then split the recorded data into the 7 different scenarios based on the turning signal and front 60$^o$FOV camera data.  }
    \end{tabular}
\end{table}
